Survey on Strategic Mining in Blockchain: A Reinforcement Learning Approach

Strategic mining attacks, such as selfish mining, exploit blockchain consensus protocols by deviating from honest behavior to maximize rewards. Markov Decision Process (MDP) analysis faces scalability challenges in modern digital economics, including blockchain. To address these limitations, reinforcement learning (RL) provides a scalable alternative, enabling adaptive strategy optimization in complex dynamic environments. In this survey, we examine RL's role in strategic mining analysis, comparing it to MDP-based approaches. We begin by reviewing foundational MDP models and their limitations, before exploring RL frameworks that can learn near-optimal strategies across various protocols. Building on this analysis, we compare RL techniques and their effectiveness in deriving security thresholds, such as the minimum attacker power required for profitable attacks. Expanding the discussion further, we classify consensus protocols and propose open challenges, such as multi-agent dynamics and real-world validation. This survey highlights the potential of reinforcement learning (RL) to address the challenges of selfish mining, including protocol design, threat detection, and security analysis, while offering a strategic roadmap for researchers in decentralized systems and AI-driven analytics.

==> Sections/Old_version/1-Introduction.tex <==
\section{Introduction}

%blockchain technique cryptocurrency: block contains transactions and participants' incentive/consensus mechanism
In recent years, blockchain technology has been widely applied to handle problems in various domains, developing innovative solutions in ways that have not been considered possible in the past.
It all started with an inventive ledge design to record all transactions generated in a decentralized system called bitcoin, invented by~\cite{nakamoto2008bitcoin}. 
This revolutionary ledger design maintains a sequentially growing list of blocks, each containing several transactions and linked with a preceding block with cryptographic techniques. 
The process of adding new blocks is governed by a consensus mechanism called Proof of Work, in which miners are rewarded with newly minted bitcoins.
This mechanism secures the network from malicious threats and stabilizes the rate of block creation, ensuring steady transaction processing. 
As a result, a permissionless and incentivized cryptocurrency system is established.

%A standout innovation of Bitcoin is its use of the consensus mechanism known as Proof of Work (PoW), where participants should complete the right to add new blocks by solving cryptographic puzzles.
%The first miner to resolve the puzzle receives newly minted bitcoins and transaction fees as rewards.
%This mechanism secures the network from malicious threats and stabilizes the rate of block creation, ensuring steady transaction processing. 
%Moreover, as long as participants act honestly, their expected earnings correlate directly with their computational power.

%下面是不是要说矿工incentive problem
Following this, numerous blockchain-based cryptocurrency protocols have been proposed, yet all participants face a common block competition issue.
For the convenience of readers, we choose a simple setting where each participant of the distributed system has its own account.
A transaction is either a creation of a fixed number of tokens assigned to the block miner, or a certain number of tokens switched hands. 
The owner of an account aims to optimize the total number of tokens in its account. 
The system is consistent if each transaction, supposedly known only to the involved participants, becomes the common knowledge of all.  

The problem cannot be reduced to a broadcast problem because of an incentive complication: 
Each participant may not be truthful if lying can bring in more tokens than executing the broadcast protocol honestly. 
It is one of the most fundamental problems in the study of distributed systems, as well as multi-agent systems. 

%multi-agent, MDP problem, Stocastic game. 有incentive, thus security problem become a game problem.

%Selfishmining is MDP strategy.

%Blockchain economic problem = solving game.

In the design of the consensus protocol
of the pioneering blockchain ecosystem, bitcoin \cite{nakamoto2008bitcoin} 
created a decentralized electronic payment system, operating without intermediaries or trusted third parties.
This marks a significant departure from traditional financial systems, offering a novel approach to secure transactions and store value in a distributed manner, across a network of nodes. 
%Each transaction is cryptographically linked to the preceding one, forming a chain of blocks, hence the term "blockchain". 
This design ensures immutability and transparency. 

A standout innovation of Bitcoin is its use of the consensus mechanism known as Proof of Work (PoW), where participants should complete the right to add new blocks by solving cryptographic puzzles.
The first miner to resolve the puzzle receives newly minted bitcoins and transaction fees as rewards.
This mechanism secures the network from malicious threats and stabilizes the rate of block creation, ensuring steady transaction processing. 
Moreover, as long as participants act honestly, their expected earnings correlate directly with their computational power.

%Bitcoin makes use of a consensus mechanism known as Proof of Work (PoW) to validate and to add a new block a step by a step to the blockchain. 

%In the PoW protocol, miners compete to solve complex mathematical puzzles. 
%The first miner to find a valid solution is rewarded with newly minted bitcoins and transaction fees. 
%This process secures the network against malicious actors and regulates the block creation rate, maintaining a consistent transaction throughput.
%Meanwhile, so long as all participants behave honestly in this system, one's expected revenue will be proportional to its computational power.


As the pioneering blockchain ecosystem, bitcoin \cite{nakamoto2008bitcoin} introduced a decentralized electronic payment system, operating without intermediaries or trusted third parties.
This marked a significant departure from traditional financial systems, offering a novel approach to secure transactions and store value in a distributed manner.
The concept of blockchain, as introduced by Bitcoin, revolves around a decentralized ledger that records all transactions across a network of nodes. 
Each transaction is cryptographically linked to the preceding one, forming a chain of blocks, hence the term "blockchain". 
This design ensures immutability and transparency. 
Altering any past transaction would require consensus from most network participants, making it computationally infeasible to tamper with the data.
%
% blockchain consensus and mining strategy
To maintain transaction execution, Bitcoin employs a consensus mechanism known as Proof of Work (PoW) to validate and add new blocks to the blockchain. 
In the PoW protocol, miners compete to solve complex mathematical puzzles. 
The first miner to find a valid solution is rewarded with newly minted bitcoins and transaction fees. 
This process secures the network against malicious actors and regulates the block creation rate, maintaining a consistent transaction throughput.
Meanwhile, so long as all participants behave honestly in this system, one's expected revenue will be proportional to its computational power.
%
% Safety and security issues on blockchain consensus problem and miner's strategies behaviors.
However, in practice, miners are rational and may act strategically to get more revenue.
\cite{eyal2014majority} firstly proposed a mining strategy called Selfish mining, in which miners can strategically hide and propose the block to maintain more mining profits.
This indicates that the Bitcoin mining protocol is not incentive-compatible.
The key idea behind the attack is to induce honest miners to waste
their mining power. 
As a result, the selfish pool could obtain more revenue than its fair share.
Because of this, many researchers have studied the safety and security problems of consensus protocols and achieved some results.
%
% Our contribution
In this paper, we present a comprehensive survey focusing on the safety and security aspects of blockchain consensus protocols and their related concepts.
The rest of the paper is organized as follows:
% 别人做的哪些，以及把我们要做的放进去衔接起来。

% Open problem: 
% 1 Multi-agent情景，可以做insightful mining。
% 2 安全指标和度量框架
% 3 延迟的模型刻画
% 在这篇论文中，我们系统性得整理了区块链中策略性挖矿，以及其对共识安全影响的相关研究。同时，我们也

==> Sections/Old_version/2-Consensus.tex <==
\section{Consensus and Strategic Mining}
% intro里面的一些拿过来？

\subsection{SM MDP}

Formally, if all other participants are following the standard protocol, the attacker faces a single-player decision problem of the form $M := <S, A, P, R>$, where $S$ is the state space, $A$ the action space, $P$ a stochastic transition matrix that describes the probability of transitioning between states, and $R$ the reward matrix. Though similar in structure, we do not regard $M$ as an MDP, since the objective function is nonlinear: The player aims to maximize its share of the accepted blocks, rather than the absolute number of its own accepted ones; its goal is to have a greater return-on-investment than its counterparts

\textbf{Action space}
Actions. We begin with the description of the action space A, which will motivate the nontrivial construction of the state space.
\begin{itemize}
    \item Adopt. The action \emph{adopt} is always feasible, and represents the attacker’s acceptance of the honest network’s chain. The $a$ blocks in the attacker’s current chain are discarded.
    \item Override. The action \emph{override} represents the publication of the attacker’s blocks, and is feasible whenever $a > h$.
    \item Match. This action represents the case where the most recent block was built by the honest network, and the attacker now publishes a conflicting block of the same height. This action is not always feasible (the attacker must have a block prepared in advance to execute such a race). The statespace explicitly encodes the feasibility status of this action (see below).
    \item Wait. Lastly, the wait action, which is always feasible, implies that the attacker does not publish new blocks, but keeps working on its branch until a new block is built.
\end{itemize}

\textbf{State space}
The state space, denoted $S$, is defined by 3-tuples of the form $(a, h, fork)$. The first two entries represent the lengths of the attacker’s chain and the honest network’s chain, built after the latest fork (that is, above the most recent block accepted by all). The field fork obtains three values, dubbed irrelevant, relevant and active. State of the form $(a, h, relevant)$ means that the previous state was of the form $(a, h - 1, \cdot)$; this implies that if $a \geq h$, match is feasible. Conversely, $(a, h, irrelevant)$ denotes the case where the previous state was $(a - 1, h, \cdot)$, rendering match now ineffective, as all honest nodes received already the $h$’th block. The third label, active, represents the case where the honest network is already split, due to a previous match action; this information affects the transition to the next state, as described below. We will refer to states as $(a, h)$ or $(a, h, \cdot)$, in contexts where the fork label plays no effective role.

\textbf{Reward}
In order to keep the time averaging of rewards in scale, every state transition corresponds to the creation of a new block. The initial state $X_0$ is $(1, 0, irrelevant)$ w.p. $\alpha$ or $(0, 1, irrelevant)$ w.p. $(1 - \alpha)$. Rewards are given as elements in $N^2$, where the first entry represents blocks of the attacker that have been accepted by all parties, and the second one, similarly, for those of the honest network.

The transition matrix $P$ and reward matrix $R$ are succinctly described in Table. Largely, an adopt action “resets” the game, hence the state following
it has the same distribution as $X_0$; its immediate reward is $h$ in the  coordinate corresponding to the honest network. An override reduces the attacker’s secret chain by $h+1$ blocks, which it publishes, and which the honest network accepts. This bestows a reward of $h + 1$ blocks to the attacker. The state following a match action depends on whether the next block is created by the attacker $(\alpha)$, by honest nodes working on their branch of the chain $((1 - \gamma) \cdot (1 - \alpha))$, or by an honest node which accepted the sub-chain that the attacker published $(\gamma \cdot (1-\alpha))$. In the latter case, the attacker has effectively overridden the honest network’s previous chain, and is awarded $h$ accordingly.

\begin{table}[h]
\label{Table1}
\centering
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{State × Action}                    & \textbf{State}                    & \textbf{Probability}          & \textbf{Reward}  \\ \hline
$(a,h,\cdot), \text{adopt}$                & $(1,0,\text{irrelevant})$         & $\alpha$                      & $(0,h)$          \\ \cline{2-4} 
                                           & $(0,1,\text{irrelevant})$         & $1-\alpha$                    & $(0,h)$          \\ \hline
$(a,h,\cdot), \text{override}^\dagger$     & $(a-h,0,\text{irrelevant})$       & $\alpha$                      & $(h+1,0)$        \\ \cline{2-4} 
                                           & $(a-h-1,1,\text{relevant})$       & $1-\alpha$                    & $(h+1,0)$        \\ \hline
$(a,h,\text{irrelevant}), \text{wait}$     & $(a+1,h,\text{irrelevant})$       & $\alpha$                      & $(0,0)$          \\ \hline
$(a,h,\text{relevant}), \text{wait}$       & $(a,h+1,\text{relevant})$         & $1-\alpha$                    & $(0,0)$          \\ \hline
$(a,h,\text{active}), \text{wait}$         & $(a+1,h,\text{active})$           & $(\gamma) \cdot (1-\alpha)$   & $(0,0)$          \\ \hline
$(a,h,\text{relevant}), \text{match}^\ddagger$ & $(a-h,1,\text{relevant})$        & $\gamma \cdot (1-\alpha)$     & $(h,0)$          \\ \cline{2-4} 
                                           & $(a,h+1,\text{relevant})$         & $(1-\gamma) \cdot (1-\alpha)$ & $(0,0)$          \\ \hline
\end{tabular}
\caption{A description of the transition and reward matrices $P$ and $R$ in the decision problem $M$. The third column contains the probability of transiting from the state specified in the left-most column, under the action specified therein, to the state on the second one. The corresponding two-dimensional reward (the reward of the attacker and that of the honest nodes) is specified on the right-most column.}
\footnotesize{$^\dagger$feasible only when $a \geq h$}
\footnotesize{$^\ddagger$feasible only when $a \geq h$}
\end{table}

\textbf{Objective Function}
As explained in the introduction, the attacker aims to maximize its relative revenue, rather than its absolute one as usual in MDPs. Let $\pi$ be a policy of the player; we will write $\pi(a, h, fork)$ for the action that $\pi$ dictates be taken at state $(a, h, fork)$. Denote by $X^{\pi}_t$ the state visited by time $t$ under $\pi$, and let $r(x, y, \pi) = (r1(x, y, \pi), r2(x, y, \pi))$ be the immediate reward from transiting from state x to state y, under the action dictated by $\pi$. $X^{\pi}_t$ will denote the $t$’th state that was visited. We will abbreviate $r_t(X^\pi_t ,X^\pi_{t+1}, \pi)$ and write simply $r_t(\pi)$ or even $r_t$, when context is clear. The objective function of the player is its relative payoff, defined by
\begin{align}
    REV := \mathcal{E} \left[ \liminf_{T \rightarrow \infty} \frac{\sum_{t=1}^T r_t^1(\pi)}{\sum_{t=1}^T(r_t^1(\pi)+r_t^2(\pi))} \right]    
\end{align}
We will specify the parameters of REV depending on the context (e.g.,
$REV(\pi, \alpha, \gamma), REV(\pi), REV(\alpha))$, and will occasionally denote the value of $REV$ by $\rho$. In addition, for full definiteness of $REV$, we rule out pathological behaviours in which the attacker waits forever—formally, the expected time for the next non-null action of the attacker must be finite.

==> Sections/Old_version/3-MDP.tex <==
\section{Methodology}

\subsection{Markov Reward Process}

A Markov chain is a stochastic process that evolves through a sequence of states, where the probability of transitioning to the next state depends only on the current state (i.e., it has memoryless property). A Markov chain is defined by a finite or countably infinite set of states, transition probabilities between states, and an initial probability distribution over the states. 

\begin{definition}
    A Markov chain is a stochastic process $(X_t)_{t=0}^{\infty}$ with the following:
    \begin{itemize}
        \item A countable or finite state space $\{s_0, s_1, ... ,s_n\} \in S$.
        \item A transition matrix $P = (p_{ij})$, where $p_{ij}$ represents the probability of transitioning from state $s_i$ to state $s_j$.
        \item Markov property:
        $P(X_{N+1} = s_i | X_0 = s_{t_0}, X_1 = s_{t_1}, \ldots, X_{N} = s_{t_N}) = P(X_{N+1} = s_i | X_N = s_{t_N})$
    \end{itemize}
\end{definition}

%Markov chains 在区块链共识建模中有广泛的应用。 

\subsection{Reinforcement Learning}

Reinforcement learning is a class of machine learning algorithms that enables an agent to learn to make decisions or take actions in an environment to maximize a cumulative reward.
The agent learns through trial and error, receiving feedback from the environment through rewards or punishments.
Deep reinforcement learning combines reinforcement learning with deep learning techniques, using neural networks to approximate the value function or policy of the agent.
It is a suitable method to solve complex Markov Reward Process problems in which the environment responds reward to the agent's actions according to the transition probability.

There has been growing interest in applying reinforcement learning techniques, including deep reinforcement learning, to blockchain research in recent years.
%Paper description

\subsection{Security Threshold}

%define of Security Threshold


\subsection{MDP Model}
Formally, if all other participants are following the standard protocol, the attacker faces a single-player decision problem of the form $M := <S, A, P, R>$, where $S$ is the state space, $A$ the action space, $P$ a stochastic transition matrix that describes the probability of transitioning between states, and $R$ the reward matrix. Though similar in structure, we do not regard $M$ as an MDP, since the objective function is nonlinear: The player aims to maximize its share of the accepted blocks, rather than the absolute number of its own accepted ones; its goal is to have a greater return-on-investment than its counterparts

\textbf{Action space}
Actions. We begin with the description of the action space A, which will motivate the nontrivial construction of the state space.
\begin{itemize}
    \item Adopt. The action \emph{adopt} is always feasible, and represents the attacker’s acceptance of the honest network’s chain. The $a$ blocks in the attacker’s current chain are discarded.
    \item Override. The action \emph{override} represents the publication of the attacker’s blocks, and is feasible whenever $a > h$.
    \item Match. This action represents the case where the most recent block was built by the honest network, and the attacker now publishes a conflicting block of the same height. This action is not always feasible (the attacker must have a block prepared in advance to execute such a race). The statespace explicitly encodes the feasibility status of this action (see below).
    \item Wait. Lastly, the wait action, which is always feasible, implies that the attacker does not publish new blocks, but keeps working on its branch until a new block is built.
\end{itemize}

\textbf{State space}
The state space, denoted $S$, is defined by 3-tuples of the form $(a, h, fork)$. The first two entries represent the lengths of the attacker’s chain and the honest network’s chain, built after the latest fork (that is, above the most recent block accepted by all). The field fork obtains three values, dubbed irrelevant, relevant and active. State of the form $(a, h, relevant)$ means that the previous state was of the form $(a, h - 1, \cdot)$; this implies that if $a \geq h$, match is feasible. Conversely, $(a, h, irrelevant)$ denotes the case where the previous state was $(a - 1, h, \cdot)$, rendering match now ineffective, as all honest nodes received already the $h$’th block. The third label, active, represents the case where the honest network is already split, due to a previous match action; this information affects the transition to the next state, as described below. We will refer to states as $(a, h)$ or $(a, h, \cdot)$, in contexts where the fork label plays no effective role.

\textbf{Reward}
In order to keep the time averaging of rewards in scale, every state transition corresponds to the creation of a new block. The initial state $X_0$ is $(1, 0, irrelevant)$ w.p. $\alpha$ or $(0, 1, irrelevant)$ w.p. $(1 - \alpha)$. Rewards are given as elements in $N^2$, where the first entry represents blocks of the attacker that have been accepted by all parties, and the second one, similarly, for those of the honest network.

The transition matrix $P$ and reward matrix $R$ are succinctly described in Table. Largely, an adopt action “resets” the game, hence the state following
it has the same distribution as $X_0$; its immediate reward is $h$ in the  coordinate corresponding to the honest network. An override reduces the attacker’s secret chain by $h+1$ blocks, which it publishes, and which the honest network accepts. This bestows a reward of $h + 1$ blocks to the attacker. The state following a match action depends on whether the next block is created by the attacker $(\alpha)$, by honest nodes working on their branch of the chain $((1 - \gamma) \cdot (1 - \alpha))$, or by an honest node which accepted the sub-chain that the attacker published $(\gamma \cdot (1-\alpha))$. In the latter case, the attacker has effectively overridden the honest network’s previous chain, and is awarded $h$ accordingly.

\textbf{Objective Function}
As explained in the introduction, the attacker aims to maximize its relative revenue, rather than its absolute one as usual in MDPs. Let $\pi$ be a policy of the player; we will write $\pi(a, h, fork)$ for the action that $\pi$ dictates be taken at state $(a, h, fork)$. Denote by $X^{\pi}_t$ the state visited by time $t$ under $\pi$, and let $r(x, y, \pi) = (r1(x, y, \pi), r2(x, y, \pi))$ be the immediate reward from transiting from state x to state y, under the action dictated by $\pi$. $X^{\pi}_t$ will denote the $t$’th state that was visited. We will abbreviate $r_t(X^\pi_t ,X^\pi_{t+1}, \pi)$ and write simply $r_t(\pi)$ or even $r_t$, when context is clear. The objective function of the player is its relative payoff, defined by
$$
    REV := \mathcal{E} \left[ \liminf_{T \rightarrow \infty} \frac{\sum_{t=1}^T r_t^1(\pi)}{\sum_{t=1}^T(r_t^1(\pi)+r_t^2(\pi))} \right]    
$$
We will specify the parameters of REV depending on the context (e.g.,
$REV(\pi, \alpha, \gamma), REV(\pi), REV(\alpha))$, and will occasionally denote the value of $REV$ by $\rho$. In addition, for full definiteness of $REV$, we rule out pathological behaviours in which the attacker waits forever—formally, the expected time for the next non-null action of the attacker must be finite.

==> Sections/Old_version/4-Results.tex <==
\section{Results}

% 1.在基础Consensus基础上，考虑了哪些特殊的环境设计
% 2.Selfish(Strategic) miner strategy space
% 3.Honest(Other) miner's action
% 4.MDP/Learning Solving Methods or Technique
% 5.Results: security threshold, some insight to explain it.



%\begin{table*}[ht]
%\centering
%\caption{Consensus Mechanism Classification}
%\renewcommand{\arraystretch}{1.5} % Adjust row height
%\setlength{\tabcolsep}{5pt} % Adjust column spacing
%\begin{tabular}{|p{3cm}|p{3cm}|p{5cm}|p{6cm}|}
%\hline
%\multicolumn{2}{|c|}{\textbf{Category}} & \multicolumn{1}{c|}{\textbf{Consensus Protocols}} & \multicolumn{1}{c|}{\textbf{Description}} \\ \hline
\multicolumn{1}{|c|}{}                                    & Longest Chain Rule  & Bitcoin\cite{nakamoto2008bitcoin}, Ethereum 1.0\cite{wood2014ethereum}, FruitChain\cite{pass2017fruitchains}                        & Based on PoW, selecting the longest chain by computational work. \\ \cline{2-4}
\multicolumn{1}{|c|}{\multirow{-2}{*}{Chain-based Rules}} & Heaviest Chain Rule & Ouroboros\cite{kiayias2017ouroboros}, PoST \cite{moran2019simple} & Based on PoS or storage, selecting the chain with the highest accumulated weight. \\ \hline
\multicolumn{2}{|c|}{Vote-based Rules}                                          & PBFT\cite{castro1999practical}, Tendermint \cite{buchman2016tendermint}, Diem BFT \cite{team2021diembft}, HotStuff\cite{yin2019hotstuff}, Ethereum 2.0\cite{buterin2020combining} & Deterministic consensus with a voting mechanism, ensuring finality without forks and randomness. \\ \hline
\multicolumn{2}{|c|}{Parallel Confirmation Rules}                                           & Avalanche \cite{rocket2019scalable}, Sui \cite{blackshear2023sui} & Probabilistic consensus based on DAG, supporting high throughput and scalability. \\ \hline
\end{tabular}
\end{table*}


\subsection{Proof of Work Consensus}

\textbf{Selfish mining} - Jichen Li
It has long been believed that the Bitcoin protocol is incentive-compatible. However, Eyal and Sirer~\cite{eyal2014majority} indicate this is not the case. It describes a well-known attack called selfish mining. A pool could receive higher rewards than its fair share via the selfish mining strategy. This attack ingeniously exploits the conflict-resolution rule of the Bitcoin protocol, in which when encountering a fork, only one chain of blocks will be considered valid. With the selfish mining strategy, the attacker deliberately creates a fork and forces honest miners to waste efforts on a stale branch. Specifically, the selfish pool strategically keeps its newly found block secret rather than publishing it immediately. Afterward, it continues to mine on the head of this private branch. When the honest miners generate a new block, the selfish pool will correspondingly publish one private block at the same height and thus create a fork. Once the selfish pool's leads are reduced to two, an honest block will prompt it to reveal all its private blocks. As a well-known conclusion, assuming that the honest miners apply the uniform tie-breaking rule, if the fraction of the selfish pool's mining power is greater than $25\%$, it will always get more benefit than behaving honestly.

\textbf{Optimal Selfish mining} - Jichen Li
\cite{sapirshtein2016optimal} extend the underlying model for selfish mining attacks, and provide an algorithm to find Q-optimal policies for attackers within the model, as well as tight upper bounds on the revenue of optimal policies. 
As a consequence, the algorithm are able to provide lower bounds on the computational power an attacker needs in order to benefit from selfish mining. 
Paper find that the profit threshold – the minimal fraction of resources required for a profitable attack – is strictly lower than the one induced by the \cite{eyal2014majority} scheme. Indeed, the policies given by our algorithm dominate orginal selfish mining strategy, by better regulating attack-withdrawals.

\textbf{A Better Method to Analyze Blockchain Consistency} - Jichen Li
When considering how to analyze a PoW blockchain protocol, the formal frameworks only analyze the consistency and liveness of the chain.
Paper \cite{kiffer2018better} provides a Markov-chain based method for analyzing the consistency properties of blockchain protocols.
They consider a partially synchronous network that proposed blocks in the rounds and an adaptive corrupt adversary.
The adversary can break blockchain consistency by processing a family of delaying attacks, in which they will withhold their block and broadcast it when any honest miner finds a block.
By analyzing this attack, the authors show strong concentration bounds to demonstrate how long a participant should wait before considering a high-value transaction to be confirmed.

\textbf{Lay Down the Common Metrics: Evaluating Proof-of-Work Consensus Protocols’ Security} - Binfeng Song, Lijia Xie
\cite{zhang2019lay} employed a multi-metric evaluation framework based on Markov decision processes to quantitatively assess the chain quality and attack resistance of several existing enhanced PoW protocols. In this framework, the metric of incentive compatibility serves as an indicator of a protocol's resistance to selfish mining.
In the analysis of selfish mining strategies using MDP modeling, 
selfish miners can secretly withhold their discovered blocks, revealing their chain only when it surpasses the length of the public chain or when their lead is reduced to a single block. Conversely, honest miners adheres to protocol rules, promptly publishing blocks and choosing the longest chain for mining. The conclusions suggest that current enhanced PoW protocols fail to achieve optimal chain quality or robust attack resistance. This shortfall is attributed to the inherent dilemma in existing protocols between rewarding malicious actions and penalizing adherence to the protocol.

\textbf{SquirRL} - Wanying Zeng, Bo Zhou
\cite{hou2019squirrl} introduce SquirRL, a framework that leverages deep reinforcement learning to explore vulnerabilities in blockchain incentive mechanisms and recover adversarial strategies. Application of SquirRL successfully uncovers previously known attacks, including the optimal selfish mining attack in Bitcoin \cite{sapirshtein2016optimal}, and the Nash equilibrium in block withholding attacks\cite{eyal2015miner}. 

SquirRL applies to selfish-mining evaluation in blockchain consensus/incentive protocols through the following steps:
(a)Environment Construction: The environment involves features and action spaces reflecting the views and capabilities of participating agents. SquirRL considers different environment designs, including single selfish miner, and multiple selfish miners, as well as dynamic and stochastic environment designs, on top of the basic consensus protocol.
(b)Adversarial Model Selection: The protocol designer selects an adversarial model, including the numbers and types of agents, to explore various adversarial strategies.
(c)RL Algorithm Selection: The protocol designer selects an RL algorithm appropriate for the environment and adversarial model, associating it with a reward function and hyperparameters. SquirRL utilizes deep reinforcement learning (DRL) algorithms to solve Markov Decision Processes (MDPs), including both value-based methods and policy gradient methods.
(d)Training and Evaluation: SquirRL trains DRL agents in the selected environment and evaluates the performance of various strategies, including selfish mining, against baseline strategies and known theoretical results.

The paper yields novel empirical insights. Firstly, a counterintuitive flaw is identified in the widely used rushing adversary model when applied to multi-agent Markov games with incomplete information.
Secondly, contrary to previous assumptions, the optimal selfish mining strategy identified in \cite{sapirshtein2016optimal} is not a Nash equilibrium in the multi-agent selfish mining context. The results suggest (though not conclusively proven) that when more than two competing agents engage in selfish mining, no profitable Nash equilibrium exists. This observation aligns with the lack of observed selfish mining behavior in real-world scenarios.
Thirdly, a novel attack is uncovered on a simplified version of Ethereum’s finalization mechanism, Casper the Friendly Finality Gadget (FFG). This attack allows a strategic agent to amplify her rewards by up to 30\%.


\textbf{WeRLman} - Hanting Huang, Nuojing Liang
Incentives are crucial to ensuring the security of proof-of-work blockchain protocols. In the operation of blockchain systems, whale transactions, characterized by offering additional transaction costs, occur occasionally. WeRLman is the first selfish-mining analysis model considering both subsidy and transaction fees\cite{bar2022werlman}. Like Squirl, WeRLman describes blockchain through a Markov Decision Process (MDP). To cope with the complexity of the model and the large policy space, WeRLman utilizes a deep reinforcement learning framework inspired by the principles of AlphaGo Zero and incorporates Monte Carlo Tree Search (MCTS) and Deep Q Network (DQN) methods. Through experiments extracted from the Bitcoin platform data, analysis based on WeRLman reveals a clear inverse relationship between fee changes and the system security threshold. It is worth noting that the security threshold is considerably lower in the case of whale transactions compared to the security threshold of 0.25 analyzed by the previous model built under constant rewards. Specifically, based on Bitcoin's historical fees with its minting strategy, the deviation thresholds would be reduced to 0.2 in 10 years, 0.17 in 20 years, and 0.12 in 30 years. Based on the current transaction costs of the Ethernet smart contract platform, the security threshold would be reduced to 0.17, which is below the common sizes of large miners.

\textbf{Deep Bribe: Predicting the Rise of Bribery in Blockc-hain Mining with Deep RL} - Jiawei Nie, Feifan Wang 
\cite{bar2023deep}Building upon WeRLman, the article further considers the impact of petty compliant miners on the security threshold. Specifically, as transaction fees relative to the block's inherent reward (BTC) gradually increase, some miners tend to favor chains with more transaction fees when producing forks, leading to the emergence of undercutting attacks. In this environment, selfish miners can attract petty compliant miners to mine on their forked chain by creating equally long chains with lower transaction fees, resulting in a lower security threshold. For the MDP Solving Method, PTO is first used for MDP transformation, followed by WeRLman for solving (based on MCTS and DQN). In the model of this article, when the proportion of petty compliant miners $\beta\geq$  0.75, the obtained security thresholds are respectively below 0.19 (additional transaction fee F = 0.14) and 0.13 (F = 0.74). This reflects that when considering the MEV represented by transaction fee differences, undercutting attacks (or bribery) can exacerbate the threat of selfish mining.

\textbf{Insightful Mining} - Jichen Li
In this paper, first, we propose a novel strategy called insightful mining to counteract the selfish mining attack. 
By infiltrating an undercover miner into the selfish pool, the insightful pool could acquire the number of its hidden blocks.
We prove that, with this extra insight, the utility of the insightful pool is strictly greater than the selfish pool’s when they have the same mining power. 
Then we investigate the mining game where all pools can choose to be honest or take the insightful mining strategy. 
We characterize the Nash equilibrium of such a game and derive three corollaries: 
(a) each mining game has a pure Nash equilibrium; 
(b) there are at most two insightful pools under some equilibrium no matter how the mining power is distributed; 
(c) honest mining is a Nash equilibrium if the largest mining pool has a fraction of mining power no more than 1/3.
Our work explores, for the first time, the idea of spying in the selfish mining attack, which might shed new light on researchers in the field.

\textbf{Undetectable Selfish Mining} - Feifan Wang, Jichen Li
\cite{bahrani2023undetectable}This paper builds upon the selfish mining model proposed by Eyal and Sirer\cite{eyal2014majority}, introducing the concept of statistically detectable actions and designing selfish mining strategies that achieve statistical undetectability. Firstly, the paper extends the Nakamoto Consensus Game (NCG) to l-NCG by introducing a delay parameter, innovatively characterizing the natural occurrence rate and statistical distribution of orphan blocks using this delay parameter. Subsequently, the paper demonstrates that two classical selfish mining strategies—Selfish Mining and Strong Selfish Mining—are statistically detectable due to the presence of strategic players, which leads to non-independent and non-identically distributed probabilities of generating orphan blocks at different heights. Then, starting from Selfish Mining and Strong Selfish Mining, it achieves undetectability by modifying the block publication method while ensuring strict profitability. Specifically, strategic players devise appropriate Labeling Strategy and Broadcasting Strategy based on the state of the previous height, ensuring that the probability of generating orphan blocks at the next height remains constant at a specified value. Through simple mathematical derivation and exact MDP solutions verification, the paper indicates that when the hash rate of strategic players exceeds 0.382, suitable strategies can always be found to achieve additional profits in the sense of statistical undetectability.


\subsection{Proof of Stake Consensus}
\textbf{Deep Selfish Proposing in Longest-Chain Proof-of-Stake Protocols} - Hanting Huang, Qingmao Yao

Though the longest chain rule was originally designed for features of the proof-of-work (PoW) protocol, some PoS-based blockchain protocols have also adopted it as their consensus protocol. However, there is no mining process in PoS; instead, there is the election of proposers. The selfish mining attack is one of the most important threats that can undermine the longest-chain blockchain protocol. Not only PoW-based blockchains but also POS-based blockchains using the longest chain paradigm face the threat of selfish mining. Since POS-based blockchains do not involve a mining process, the term "selfish proposing" is used instead of selfish mining to describe this attack. Compared to PoW protocols, generating valid blocks in LC-PoS is effortless. Based on the phenomenon called nothing-at-stake, attackers can expand their attacking strategies and generate new attack actions. Also, PoS protocols suffer from a degree of predictability for the lottery mechanism that specifies the block proposer(s) for each slot. This work \cite{sarenche2024deep} considers the selfish proposing attack in the longest-chain PoS (LC-PoS) blockchains. By generalizing the nothing-at-stake selfish proposing attack with different levels of predictability, it is concluded that the proposing block ratio will be slightly increased with the Nothing-at-Stake phenomenon, and proposer predictability will considerably increase the attack block ratio. To analyze the selfish proposing attack in more complicated scenarios, this work uses a Deep Q-learning tool to analyze the selfish proposing attack and obtain the near-optimal attack strategy with varying stake shares.

\textbf{Formal Barriers to Longest-Chain Proof-of-Stake Protocols} - Lijia Xie, Binfeng Song

In the study by \cite{brown2019formal}, a model for PoS (Proof of Stake) cryptocurrencies was proposed to analyze security issues driven by incentives. The paper establishes two key properties: predictability and recency, ensuring that every protocol within the model satisfies at least one of these properties. Moreover, the security implications of predictability and recency indicate that every protocol is vulnerable to at least one type of attack, including selfish mining, double spending, or Nothing-at-Stake attacks. In contrast to the adversarial corruption found in PoW (Proof of Work) systems, the main findings of this paper highlight the formal barriers to designing incentive-compatible PoS cryptocurrencies, stemming from the inherent pseudorandomness of PoS systems.

\textbf{Optimal Strategic Mining Against Cryptographic Self-Selection in Proof-of-stake} - Bo Zhou, Wanying Zeng

The paper \cite{ferreira2022optimal} considers an adversary who aims to lead and win in the PoS election protocol, maximizing the number of rounds they can win, and indicates that the presence of an adversary can gain more benefits through strategy, regardless of the proportion of stacks they control. In the Cryptographic self-selection protocol, a leader needs to be elected for each round to generate blocks, and the election of the leader is related to the stakes held by the players and the seeds of current round of. The leader can generate biased seeds to make them advantageous in subsequent rounds of elections. Ferreira et al. showed that when the stack ratio mastered by strategy players is less than 0.38, they can win at most one round. They also proposed a 1-Lookahead strategy that can strictly outperform any honest strategy under any stack ratio. Finally, they proposed an algorithm to find the optimal strategy through MDP.

\section{Conclusion and Discussion}



==> Sections/Old_version/5-Conclusion.tex <==
\section{Conclusion and Open Problems}

In this section, we introduce the blockchain system model and give an overview of different types of blockchain consensus.

\subsection{System Model of Blockchain}
The blockchain is a continuously growing ledger composed of records known as blocks, which are interlinked through cryptographic mechanisms. 
Each block contains a cryptographic hash of the previous block, a timestamp, and transaction data typically structured in a Merkle tree. 
This architecture ensures the blockchain's resilience against unauthorized data modifications while providing transparent and traceable information accessible to all participants. 
Essentially, the blockchain operates as a decentralized and shared database, where each participant maintains a copy of the ledger, ensuring consensus and data integrity across the network.

A block within the blockchain is divided into two main components: the block header and the block body. 
The block header includes critical elements such as the version number, timestamp, target hash bits, nonce, hash value of the preceding block, and the Merkle root, which represents the cryptographic summary of all transactions within the block. 
The block body, on the other hand, contains the transactional details. Each block is cryptographically linked to its predecessor, creating a chain that allows any node within the distributed network to continuously verify the integrity of the entire blockchain. 
This linkage not only secures the data but also enables the blockchain's decentralized nature, where no single entity has control, and all participants can independently validate the blockchain's integrity.

\subsection{Proof-based Consensus}

The miner granted the privilege of block validation integrates the new block into the existing chain, thereby extending the blockchain. 

This process results in the formation of the longest main chain, stretching from the Genesis block to the most recent one, effectively recording the comprehensive history of blockchain transactions.

\subsection{Byzantine-based Consensus}

In the early studies, the consensus protocol was mainly aimed at solving the problem of reaching an agreement among nodes in the distributed system (\cite{lamport1982byzantine,fischer1985impossibility,biely2011synchronous}. 
With the emergence of malicious nodes, the focus of consensus research is gradually developing towards Byzantine fault-tolerant protocol
\cite{castro1999practical,castro2022practical,cachin2001secure}. 
The blockchain, especially the public blockchain, must adopt the BFT consensus protocol because the system needs to resist the attack of malicious nodes, while the consortium blockchain and the private
blockchain can use the Byzantine fault-tolerant or crash fault-tolerant protocols because of the strict access mechanism for the nodes.


% 之后用一两句话总结我们看过的Consensus，简单总结+突出各自的特点。
% TBFT - 宋斌峰
Tendermint BFT, as a consensus algorithm within the Byzantine Fault Tolerant (BFT) category, distinguishes itself from the conventional Practical Byzantine Fault Tolerance (PBFT) by introducing innovative mechanisms aimed at enhancing the system's security and efficiency. Through the implementation of a precommit confirmation rule requiring assent from over two-thirds of participants, TBFT maintains its ability to effectively thwart the submission of malicious blocks even in scenarios where more than one-third of nodes are Byzantine. Furthermore, TBFT places a significant emphasis on a stake-weighted voting mechanism, aligning voting power directly with the economic stakes of nodes, thereby augmenting the network's decentralization and security. By adopting a weak synchrony model and incorporating timeout procedures, TBFT ensures high efficiency and practicality when confronted with network delays and node failures, thus exemplifying superior performance in sustaining the stable operation of blockchain networks.\cite{buchman2016tendermint}

% Maxbft - 曾婉莹
Another BFT-based consensus, MaxBFT,  is an optimized three-phase BFT consensus protocol for ChainMaker. It achieves high fault tolerance while ensuring system security, efficiency, and eventual consistency. In comparison to other BFT algorithms, MaxBFT introduces several optimizations. 
Notably, it streamlines the voting process, and simplifies the three-phase consensus message types (proposal and vote messages), reducing communication complexity. 
Besides, communication occurs in a star-shaped network, minimizing message propagation and reducing network communication overhead to \(O(n)\). 
Additionally, MaxBFT decouples liveness rules from safety rules, which enhances flexibility.\cite{yin2019hotstuff}
% DPoS - 梁诺靖

% Avalanche - 谢丽佳
Avalanche\cite{rocket2019scalable} employs network subsampling to design its consensus mechanisms, where nodes repeatedly select a small group of nodes at random to converge on a common bivalent state. 
Unlike traditional BFT-based and Nakamoto mechanisms, leaderless BFT protocols in Avalanche maintain probabilistic safety guarantees without requiring global communication or precise participant knowledge. 
Avalanche leverages DAG structure to facilitate concurrent operations, achieving high throughput and scalability while compromising strict consistency to some extent.

% Diem BFT - 李济宸
Diem BFT\cite{team2021diembft}
DiemBFT designs a novel leader election mechanism that achieves leader utilization. That is, the number of times a crashed leader is elected as leader is bounded. 
Second, DiemBFT changes leaders when they are considered faulty. The previous version used the HotStuff linear view change mechanism to replace faulty leaders.
DiemBFT embraces this design choice and adopts a quadratic view-change of failed leaders, which enables it to commit blocks in two steps instead of three in the steady state.
Introduce a leader reputation mechanism that provides leader utilization under crash faults while making sure that not all committed blocks are proposed by Byzantine leaders.

% PoST - 周波
The PoST (Proof of Space and Time) consensus \cite{moran2019simple} is different from other proof-of-work mechanisms in that it consumes a lot of computing power to compete to obtain block rewards. It is mainly used to build decentralized storage networks. In the PoST consensus, miners provide storage space to obtain incentive distribution, and the miner's mining efficiency is related to the miner's storage activity. In a blockchain network built on PoST, miners can obtain tokens by providing storage, and customers can hire miners to store data by spending tokens. The big difference here is that miners aren't just keeping the blockchain running, they're also providing storage services.

% Arweave, Everfinance - 陈宏崟

\subsubsection{DAG-based Consensus}

% Sui - 黄瀚霆，王菲帆
LUTRIS\cite{blackshear2023sui} is the basic protocol of the smart-contract platform Siu, which combines DAG-based consensuses with consensus-less approaches, thus allowing it to achieve high throughput paired with valuable features such as low latency and long-term stability. 
In its design, DAG-based consensus protocols such as Narwhale\cite{danezis2022narwhal} and Bullshark\cite{spiegelman2022bullshark} can realize massive concurrency of transactions, thus achieving the design goal of high throughput. 
However, DAG-based protocols introduce a certain amount of latency, and consensus-free protocol designs such as FastPay\cite{baudet2020fastpay} serve an important role in reducing latency to increase scalability.The combination of the two types of approaches achieves superior performance metrics of sub-second latency and sustained throughput of thousands of transactions per second.

%Maybe have others
